On the role of laminar/turbulent interface on energy transfer between scales in bypass transition

We investigate the role of laminar/turbulent interface in the interscale energy transfer in a boundary layer undergoing bypass transition, with the aid of the Karman-Howarth-Monin-Hill (KHMH) equation. A local binary indicator function is used to detect the interface and employed subsequently to define two-point intermittencies. These are used to decompose the standard-averaged interscale and interspace energy fluxes into conditionally-averaged components. We find that the inverse cascade in the streamwise direction reported in an earlier work arises due to events across the downstream or upstream interfaces (head or tail respectively) of a turbulent spot. However, the three-dimensional energy flux maps reveal significant differences between these two regions: in the downstream interface, inverse cascade is stronger and dominant over a larger range of streamwise and spanwise separations. We explain this finding by considering a propagating spot of simplified shape as it crosses a fixed streamwise location. We derive also the conditionally-averaged KHMH equation, thus generalising similar equations for single-point statistics to two-point statistics. We compare the three-dimensional maps of the conditionally-averaged production and total energy flux within turbulent spots against the maps of standard-averaged quantities within the fully turbulent region. The results indicate remarkable dynamical similarities between turbulent spots and the fully turbulent region for two-point statistics. This has been known only for single-point quantities, and we show here that the similarity extends to two-point quantities as well.

==> literature_review/replace.tex <==
\chapter{Standard KHMH analysis of bypass transition}\label{Pub_2}

The success of KHMH in describing the complex interscale dynamics of near-wall turbulence justifies the adoption of this framework to explore similar issues in bypass transition. As explained earlier, the equation is very general, and therefore applicable in laminar, transitional and fully turbulent regimes. Thus, it can be employed across the laminar-turbulent interface, allowing us to get a unique glimpse of the inter-scale energy transfer process in transitional flows. In this section, The Karman-Howarth-Monin-Hill (KHMH) equation is employed to study the production and interscale energy transfer in a boundary layer undergoing bypass transition due to free-stream turbulence. The energy flux between different length scales is calculated at several streamwise locations covering the laminar, transitional, and turbulent regimes. Maps of scale energy production and flux vectors are visualised on two-dimensional planes and three-dimensional hyperplanes that comprise both physical and separation spaces. We will study the spatial evolution of the interscale energy fluxes at 6 locations, placed in the laminar $(LA)$, transitional $(TR0,TR1,TR2,TR3)$ and fully turbulent $(TA)$ regions; these locations are shown in the right panel of figure \ref{one-point Cf}. Note that in this section the numbering of the streamwise location is different from section \ref{Pub_1}. 

\begin{figure}
 \centering
    \includegraphics[scale=0.45]{Chapter5_paper2/Cf_all.png}
    \caption{Skin friction coefficient, $C_f$, against $Re_{\theta}$ (left panel) and distance from the inlet of the domain, $(X-X_0)/L_0$ (right panel). The green and black vertical lines denote locations at the laminar $(LA)$ and turbulent $(TU)$ regions respectively. The purple vertical lines denote 4 stations $TR0,TR1,TR2,TR3$ within the transitional region. The coordinates are  $(X-X_0)/L_0=540,1065,1215,1515,1815,2415$ for $LA,TR0,TR1,TR2,TR3 \mbox{ and }TU$ respectively.
    }
    \label{one-point Cf}
\end{figure}

\section{The budgets of the TKE equation}

Before we proceed to examine the evolution of two-point statistics using the KHMH equation, it is instructive to examine first the budgets of the turbulent kinetic energy (TKE) equation at these 6 locations (as the TKE equation is the asymptotic form of the KHMH equation at large scale). Figure \ref{fig:TKE_BUDGET} shows the evolution of the budget terms plotted against the distance from the wall for all streamwise positions; variables are normalised using the local wall units. The open symbols represent the reference DNS data of \cite{spalart1988direct} and are repeated in every panel. The matching between the present results at the $TU$ region (where $Re_{\theta}=800$) and the reference data (where $Re_{\theta}=1410$) is very good for all terms. This provides further evidence of the validity of the generated database. Comparison between the lines and symbols indicates the deviation from the fully turbulent state at each location.

 \begin{figure} 
    \centering
   \includegraphics[trim=0 0 0 2.5, clip, scale=0.58]{Chapter5_paper2/TKE_PART1.PNG}
   \includegraphics[trim=0 0 0 2.5, clip, scale=0.58]{Chapter5_paper2/TKE_PART2.PNG}
   \includegraphics[trim=0 0 0 2.5, clip, scale=0.58]{Chapter5_paper2/TKE_PART3.PNG}
    \caption{TKE budgets at locations $LA, TR0, TR1, TR2, TR3, TU$. The symbols represent data from \cite{spalart1988direct} for $Re_{\theta}=1410$.}
    \label{fig:TKE_BUDGET}
\end{figure}

In the laminar regime ($LA$ panel), where the boundary layer is distorted by Klebanoff modes, the production term has approximately symmetric shape, peaks at $Y^+\approx 21$ and reaches a relatively small value. As the flow transitions, the production peak grows, moves closer to the wall and finally settles at $Y^+ \approx 16$ (panel TU), i.e.\ in the buffer layer. A production overshoot appears at $TR2$, which is in the middle of the transition region. At this position the maximum intermittency is about $40\%$ (refer to figure 4 of \cite{Yao_Portela_Papadakis_2020}) and grows fast indicating the rapid formation and growth of turbulent spots. \cite{Nolan_Zaki_2013} report an overshoot in the streamwise rms velocity in exactly the same position, i.e.\ when the skin friction is midway between the laminar and turbulent values. 

At $LA$, dissipation peaks within the Klebanoff mode core, but further downstream the maximum value grows, and beyond $TR1$ it settles at the wall, where it is balanced by viscous diffusion,  as expected. Turbulent diffusion has small contribution at $LA$, $TR0$ and $TR1$, but becomes very significant at $TR2$, with a sharp positive peak close to the wall at $Y^+ \approx 5$ and a shallower negative trough at $Y^+ \approx 22$. At this location, three terms dominate for $Y^+>15$, production, dissipation and turbulent diffusion. Note also the very sharp rise of dissipation close to the wall, and the important contribution of turbulent diffusion to balance it. Further downstream, at $TR3$ and $TU$, all terms settle to smaller values. 

The largest deviation from equilibrium, quantified by the difference between production and dissipation for $Y^+ > 15$, appears in $TR2$; this is the position with the largest growth of $C_f$ as evidenced in figure \ref{one-point Cf}, consistent with the rapid increase of intermittency, as mentioned earlier. At $TR3$, where $C_f$ starts to stabilise marking the end of transition, the budgets are very similar to the fully turbulent state, $TU$. In the latter state turbulence is in equilibrium, with production balancing dissipation for $Y^+ > 25$. In all locations the convection term plays a minor role. It becomes more important in $TR2$ (and less so in $TR1$) for $Y^+ > 60$, where it balances production, dissipation and turbulent diffusion.   

 \begin{figure} 
    \centering
  \includegraphics[scale=0.6]{Chapter5_paper2/TKE_fourth.png}
    \caption{Contour plots of (a) turbulent kinetic energy, (b) production, (c) turbulent diffusion, and (d) dissipation. All variables normalised with global units. The red dashed line indicate the location of the boundary layer thickness.
    }
    \label{fig:TKE_contour}
\end{figure}

The strong wall-normal and streamwise inhomogeneity are  more clearly demonstrated in the contour plots of TKE, production, turbulent transport, and dissipation shown in figure \ref{fig:TKE_contour}, where all terms are normalized by global variables (free-stream velocity $U_\infty$, and Blasius variable at the inlet $L_0$). Turbulent kinetic energy and turbulent transport peak at $(X-X_0)/L_0 \approx 1650$, slightly downstream of $TR2$. When normalised with global variables, the production term reaches maximum in the turbulent regime. The peak of TKE therefore at $(X-X_0)/L_0 \approx 1650$ arises from the strong positive value of turbulent transport close to the wall (yellow region in panel c). Dissipation grows sharply downstream of $(X-X_0)/L_0 \approx 1600$ and is maximised at the wall. 

The TKE is one-point equation and energy is transported only in physical space. In the next section we look at the transport of energy in both physical and scale spaces using the KHMH equation.

\section{Energy fluxes on the $(r_3,Y)$ plane}\label{sec:fluxes-r3-Y}
\subsection{General characteristics}
\begin{figure} 
    \centering
%   \includegraphics[scale=0.4]{Fig/r3_flux7.png}
\includegraphics[scale=0.45]{Chapter5_paper2/r3_Y_twosinks3.PNG}
    \caption{Evolution of energy flux vector  $\left(\boldsymbol{\phi_r}_3,\boldsymbol{\phi_s}_2\right)$ on $(r_3, Y)$ plane (red arrows) from laminar to turbulent region. The coloured contour is the net production (normalised with global variables) and the pink dashed lines indicate the local boundary layer thickness. The yellow arrows at the TR2 plot point to the two sink regions, $r_3=0$ and $Y=0$. The maximum vector magnitude (corresponding to the longest  arrow on each plot) is $5\times10^{-5}, 7.6\times10^{-5}, 9.1\times10^{-5}, 1.7\times10^{-4}, 2.4\times10^{-4}, 2.2\times10^{-4}$ from $LA$ to $TU$ respectively.}
    \label{r3_flux}
\end{figure}

%Figure \ref{r3_flux} shows the evolution of the energy fluxes in the $(r_3,Y)$ plane at the 6 streamwise locations shown in figure \ref{one-point Cf}. The colour contours represent the net production $\mathcal{P}_{net}$ (normalised with global variables) while the red vectors represent the fluxes along the $r_3$ and $Y$ directions, i.e\ $({\phi_r}_3,{\phi_s}_2)$. 

Figure \ref{r3_flux} shows the evolution of the flux vector components $\left(\boldsymbol{\phi_r}_3,\boldsymbol{\phi_s}_2\right)$ in the $(r_3,Y)$ plane (with $r_1=0$) from the laminar to turbulent region. Wall-normal distances and separations are normalized by the local wall variables (left and bottom axes) and global variables (top and right axes). The pink dashed line indicates the local boundary layer thickness. In order to facilitate the interpretation of these plots, we also superimpose coloured contours of the net production, $\mathcal{P}_{net}=\mathcal{P}-\epsilon$. 

At all spatial locations $\mathcal{P}_{net}$ peaks at particular $r_3$ separations and wall-normal distances $Y$ (the peaks appear as concentrated yellow regions). The production $\mathcal{P}$ arises from the inhomogeneity of the time-average flow in the physical and scale spaces, as evidenced by the two terms in equation \eqref{eq:production}. We analysed the contribution of each term and found that the large production arises due to the inhomogeneity on scale space, and in particular from the component $-2\overline{ d u_2 d u_1 } \left. \frac{\partial d U_1}{\partial r_2}\right\vert_{r_2=0}$. The contribution of the second term is exactly 0 (due to the spanwise homogeneity of the time-average flow).  It is easier to understand the physical mechanism that leads to high production if we focus on the laminar region (top-left panel, denoted as $LA$). In this region Klebanoff modes (laminar streaks) are present that result in positive and negative streamwise velocity fluctuations, therefore $d u_1$ is maximised when $r_3$ is equal to the distance between two streaks. The wall-normal fluctuation differences $d u_2$ are also maximised at the same distance (refer to figure 24 in \cite{xiao2019nonlinear}) resulting in large time and spanwise averages $\overline{ d u_2 d u_1 }$. The shear rate in scale space can be written as $\frac{\partial d U_1}{\partial r_2}=\frac{1}{2}(\frac{\partial d U_1}{\partial x_2^+}-\frac{\partial  d U_1}{\partial x_2^-} )=
\frac{1}{2}(\frac{\partial U_1^+}{\partial x_2^+}+\frac{\partial  U_1^-}{\partial x_2^-} )$ and due to spanwise homogeneity of $U_1$ and the fact that $r_2=0$ (meaning that $x_2^+=x_2^-=x_2=Y$, thus $U_1^+=U_1^-=U_1$) this can be simplified to  $ \left. \frac{\partial d U_1}{\partial r_2}\right\vert_{r_2=0}=\frac{\partial U_1}{\partial x_2}$. The production term can therefore be written as $\mathcal{P} = -2\overline{ d u_2 d u_1 } \frac{\partial U_1}{\partial x_2}$. The corresponding term for the turbulent kinetic energy equation is $\mathcal{P}_k \approx -\overline{ u_2 u_1 } \frac{\partial U_1}{\partial x_2} $, which is of course uniform in the spanwise direction, see figure \ref{fig:TKE_contour}(b). The peak production location of the KHMH equation in the $(r_3,Y)$ plane is therefore determined by the spanwise distance between the Klebanoff modes and the wall-normal distance at which the product of the second-order structure function  $\overline{ d u_2 d u_1 }$ and the shear $\frac{\partial U_1}{\partial x_2}$ is maximum. The mean flow therefore injects energy at a specific $r_3$ separation, which is determined by the receptivity process arising from the interaction between free-stream turbulence forcing and shear during the early development of the boundary layer.  This process controls the spacing between the Klebanoff modes, which is of the order of the boundary layer thickness close to the inlet.

As the flow evolves, the location of peak net production changes smoothly and approaches the wall. The largest energy production appears at the TU location, inside the buffer layer, at $Y^+\approx 12$ and $r_3^+ \approx 40$, 
consistent with the results of \cite{cimarelli2015sources} for channel flow.  The large production at specific regions in the $(r_3,Y)$ plane strongly affects the energy transfer in the physical and scale spaces, to which we now turn.

For all streamwise locations the energy fluxes originate from the $\mathcal{P}_{net}$ peak location and radiate outwards. In the laminar region (LA), most of the energy produced flows to smaller $r_3$ scales and is dissipated (forward cascade). There is weak inverse cascade to larger $r_3$ scales, while the energy flux in the wall-normal direction is negligible. At the turbulent region (TU) the fluxes show a different behaviour. The energy injected from the time-average flow radiates in all directions. There are two sinks \textcolor{blue}{indicated by yellow arrows in the TR2 plot of figure \ref{r3_flux}}; one towards the wall (where it is dissipated) and the other towards small $r_3$ scales (indicating a forward cascade). An inverse energy cascade also appears, i.e.\ energy flows to larger $r_3$ scales to the right of the $\mathcal{P}_{net}$ before most of the flux vectors then change direction and bend towards the $Y$ axis ($r_3=0$). This map is very similar to that of turbulent channel flow \cite{cimarelli2013paths, cimarelli2016cascades, cimarelli2015sources}.

In the transition region, the scale energy transfer pattern morphs progressively from laminar to turbulent shape. Downstream of TR0, the energy flux in the wall-normal direction (i.e\ towards the bulk of the flow) energises the region above the Klebanoff modes, increasing the thickness of the boundary layer. This indicates that the equilibrium boundary layer at TU is forming gradually during the transition process. Significant inverse cascade appears towards larger $r_3$ scales, but it is noteworthy that the bending of the energy flux vectors towards small scales does not appear in the transition region, but only at the TU region. It seems that strong inverse cascade is a central characteristic of transition; we will elaborate more on this important feature again later. 

In order to shed more light into the patterns shown in figure  \ref{r3_flux}, we turn our attention to the decompositions \eqref{eq:flux_phys_space} and \eqref{eq:flux_scale_space} and investigate the contributions of fluxes due to mean flow, non-linear interactions, viscosity, and pressure.

\subsection{Analysis of decomposed energy fluxes}

\begin{figure} 
    \centering
   \includegraphics[scale=0.48]{Chapter5_paper2/TR3_yrz_FLUXall.png}
    \caption{Maps of flux vectors due to nonlinear interaction between velocity fluctuations $(F)$, viscosity $(V)$, Mean velocity $(M)$, pressure $(P)$, combination $(F+V)$, and total on $(r_3,Y)$ plane at $TR2$ location. Contours represent the magnitude of the corresponding flux vectors.}
    \label{total_flux_decomallr3}
\end{figure}

\begin{figure} 
    \centering
    \includegraphics[scale=0.45]{Chapter5_paper2/LA_yrz_decom_3.png}
    \includegraphics[scale=0.45]{Chapter5_paper2/TR0_yrz_decom_3.png}
    \includegraphics[scale=0.45]{Chapter5_paper2/TR1_yrz_decom_3.png}
    \includegraphics[scale=0.45]{Chapter5_paper2/TR2_yrz_decom_3.png}
    \includegraphics[scale=0.45]{Chapter5_paper2/TR3_yrz_decom_3.png}
    \includegraphics[scale=0.45]{Chapter5_paper2/TU_yrz_decom_3.png}
    \caption{Evolution of energy fluxes due to the non-linear interaction term (left column) and the viscous term (middle column) in the  $(r_3,Y)$ plane. The total flux is shown in the right column. Contours represent the magnitude of the corresponding flux vectors. The pink dashed line is the local boundary layer thickness.}
    \label{r3_flux_decom}
\end{figure}

We focus in particular on the $TR2$ location, in the middle of the transition region. In figure \ref{total_flux_decomallr3} we plot the four pairs of fluxes $(\boldsymbol{\phi^F_{r_3}},\boldsymbol{\phi^F_{s_2}})$, $(\boldsymbol{\phi^V_{r_3}},\boldsymbol{\phi^V_{s_2}})$, $(\boldsymbol{\phi^M_{r_3}},\boldsymbol{\phi^M_{s_2}})$ and $(\boldsymbol{0,\phi^P_{s_2}})$ in the $(r_3,Y)$ plane; these are denoted with the capital bold letters \textbf{F}, \textbf{V}, \textbf{M} and \textbf{P} respectively. We also plot the sum $\left ( \boldsymbol{\phi^F_{r_3}}+\boldsymbol{\phi^V_{r_3}},\boldsymbol{\phi^F_{s_2}}+\boldsymbol{\phi^V_{s_2}}\right)$, denoted as \textbf{F}+\textbf{V}, and the total flux $\left(\boldsymbol{\phi_r}_3,\boldsymbol{\phi_s}_2\right)$, which is of course identical to that shown in the lower left panel of figure \ref{r3_flux}. In all plots, the flux vectors are plotted as arrows to show the direction, but we also superimpose the flux magnitude as contours.  

We first note that the fluxes due to mean flow and pressure have components only in physical space, i.e.\ the wall-normal direction; this is because $ \boldsymbol{\phi^P_{r_3}}=0$ and $ \boldsymbol{\phi^M_{r_3}}=\overline{ d U_i d q^2 } =0$ due to homogeneity in the spanwise direction. Therefore in the $r_3$ direction the fluxes are due to the non-linear and viscous terms only, $ \boldsymbol{\phi^F_{r_3}}$ and $\boldsymbol{\phi^V_{r_3}}$. The latter term results in forward cascade, while the former transfers energy to larger scales (inverse cascade) and to the bulk of the flow. The superposition of these two terms results in the \textbf{F}+\textbf{V} pattern, which is almost identical to the total in the $r_3$ direction. Adding the contribution of pressure and mean flow terms, that both transfer energy towards the wall, readjusts the direction of the arrows, and completes the picture. The readjustment is especially evident at $Y \approx 5L_0$, and results in almost horizontal total inverse fluxes.

In figure \ref{r3_flux_decom} we plot the evolution of the two most important terms (viscous and non-linear) at all streamwise locations. For comparison purposes, we also include the total flux in the same plot (right column). We first notice that the viscous flux (middle column) results mainly in forward cascade (but there are some regions of very weak inverse cascade) and energy towards the wall.  As transition progresses, the  forward cascade acts at progressively smaller scales, while the energy transfer towards the wall becomes stronger. The latter is firmly established over a wide range of scales in the viscous sublayer when the turbulent region is reached. The viscous effect can be clearly seen also on the total energy flux plots, especially in the TR3 and TU locations. The energy  transfer due to non-linear interaction term is more involved. This term mainly acts to transfer energy to larger scales (inverse cascade) and this is evident at all streamwise locations, even in the laminar (LA) region (but it is quite weak there). Starting from the TR0 location, it also acts to transfer energy to the bulk of the flow. The radial flux pattern that appears in the total flux plots (right column) is thus due to the superposition of the effects of the non-linear interaction and viscous terms. 

We now turn our attention to energy transfer in the $(r_1, Y)$ plane. 

\section{Energy fluxes on the $(r_1, Y)$ plane} \label{sec:fluxes-r1-Y}
For each streamwise location, we select the $r_3$ value that corresponds to the peak net production shown in Figure \ref{r3_flux}; the resulting separations are $r_3/L_0=8,8,8,8,5,5$ at positions $LA,TR0,TR1,TR2,TR3,TU$ respectively. This allows us to investigate the behaviour of the energy fluxes in the particular $r_3$ separation at which the energy due the mean shear is injected. 

\subsection{General characteristics}

\begin{figure} 
\centering
\includegraphics[scale=0.5]{Chapter5_paper2/r1Y_crosspeak.png}
\caption{Evolution of the energy flux vector $\left(\boldsymbol{\phi_r}_1,\boldsymbol{\phi_s}_2\right)$ on $(r_1, Y)$ plane from laminar to turbulent region (red vectors). The contour values correspond to net production, and the pink dashed lines indicate the local boundary layer thickness. For $LA,TR0,TR1,TR2,TR3,TU$ locations, the separations are $r_3/L_0=8,8,8,8,5,5$ respectively; these correspond to the peak net production shown in figure \ref{r3_flux}. The maximum vector magnitude (corresponding to the longest arrow in each plot) is $5\times10^{-4}, 2.5\times10^{-4}, 6\times10^{-4}, 1\times10^{-3}, 8\times10^{-4}, 3.5\times10^{-4}$ from $LA$ to $TU$ respectively.}
\label{fig:r1Y_crosspeak}
\end{figure}

Figure \ref{fig:r1Y_crosspeak} shows the evolution of the energy flux vector $\left(\boldsymbol{\phi_r}_1, \boldsymbol{\phi_s}_2\right)$ on this plane. A core region of strong net production, indicated by yellow colour, can be clearly seen; this region persists throughout transition. At the LA location, this region is concentrated at small $r_1$ values, $0<r_1/L_0<75$, but as transition progresses, it moves closer to the wall and it is elongated. Gradually, it occupies the whole range of $r_1$ separations considered, $0<r_1/L_0<150$. Note also that apart from the first two locations $LA$ and $TR0$, net production can take negative values very close to the wall (because of strong dissipation). 

From the high production region, energy flux vectors emanate with $\boldsymbol{\phi_r}_3>0$, indicating inverse cascade. At $LA$ and $TR0$ locations this is barely noticeable, but at $TR1$ it is very strong in the region $0<r_1/L_0<100$. It is also present at the downstream locations, $TR2$, $TR3$ but at larger separations,   $75<r_1/L_0<150$, and closer to the wall. It  is very interesting to notice that once transition is complete, the inverse cascade is significantly subdued. Indeed, we can barely see it in the $TU$ region (although the strong net production region can be still seen very clearly). In the next section we probe in more depth the origin of this inverse cascade, by examining the evolution of the different components of the energy flux. 

\subsection{Decomposition of the energy fluxes.}

\begin{figure}
    \centering
 \includegraphics[scale=0.45]{Chapter5_paper2/UMEAN_all2.png}
    \caption{Contour plots of the mean streamwise velocity $U_1$ (top) and the normal strain rate $\frac{dU_1}{dX_1}$ (bottom). The black dashed curve denotes the $\frac{dU_1}{dX_1}=0$ isoline. The red dashed line indicates the boundary layer thickness.}
    \label{fig:DU1DX1}
\end{figure}

In the  $(r_3, Y)$ plane it was found that the non-linear interaction and viscous components of the energy flux were the most dominant. In the  $(r_1, Y)$ plane however, the viscous component is much less important, while energy flux due to mean flow, $\phi_{r_1}^M=\overline{ d U_1 d q^2 }$, assumes a more significant role. This is expected due to the strong streamwise inhomogeneity of the flow in the transition region. The sign of $\phi_{r_1}^M$ is determined by $d U_1$. In order to facilitate the interpretation of the results, contours of $U_1$  are shown in figure \ref{fig:DU1DX1} (top panel). For small $r_1$, $d U_1$ has the same sign as the normal strain rate $\frac{\partial U_1}{\partial x_1}$, thus contours of the latter are also shown in the figure (bottom panel). In the transition region between TR1 and TR3, a zone of accelerating flow appears close to the wall, in agreement with the rise of $C_f$ shown in figure \ref{one-point Cf}. In the laminar region the flow decelerates, with the strongest negative strain around the centre of the boundary layer.   

\begin{figure} 
    \centering
   \includegraphics[scale=0.47]{Chapter5_paper2/LA_NZr3Y_MuandFu_4.png}
   \includegraphics[scale=0.47]{Chapter5_paper2/TR0_NZr3Y_MuandFu_4.png}
   \includegraphics[scale=0.47]{Chapter5_paper2/TR1_NZr3Y_MuandFu_4.png}
   \includegraphics[scale=0.47]{Chapter5_paper2/TR3_NZr3Y_MuandFu_4.png}
   \includegraphics[scale=0.47]{Chapter5_paper2/TR5_NZr3Y_MuandFu_4.png}
   \includegraphics[scale=0.47]{Chapter5_paper2/TU_NZr3Y_MuandFu_4.png}
    \caption{Evolution of the mean (M) and non-linear interaction (F) components of the energy flux (red vectors) on the $(r_1, Y)$ plane. The contours are the magnitude of the corresponding flux vector. The spanwise separations are $r_3/L_0=8,8,8,8,5,5$ from $LA$ to $TU$ respectively.}
    \label{r1_flux_decom_crosspeak}
\end{figure}
 
The evolution of the mean (M) and non-linear interaction (F) components of the energy flux are shown in figure  \ref{r1_flux_decom_crosspeak}. Note the competition between the two components, which is quite subtle. In the laminar region LA, $d U_1<0$ and the energy flux due to the mean flow leads to forward cascade; however the non-linear interaction leads to inverse cascade. The two contributions cancel each other out, and this explains why the total flux shown in the top-left panel of figure \ref{fig:r1Y_crosspeak} is very weak for $0<r_1/L_0<75$. At $TR0$ the $C_f$ has a minimum and $d U_1 \approx 0$ for small $r_1$, but for larger separations $d U_1>0$, consistent with the steeper rise of $C_f$ at the start of transition. Again at this location the two components compete, with $\phi_{r_1}^M<0$ (forward cascade) and $\phi_{r_1}^F>0$ (inverse cascade). At TR1, $d U_1$ changes sign across the boundary layer ($d U_1<0$ away from the wall and  $d U_1\ge0$ close to it, refer to figure \ref{fig:DU1DX1}), but $\phi_{r_1}^F>0$ always, leading to overall strong inverse cascade.  At TR2 and TR3, $d U_1>0$ close to the wall and very weak further away, while $\phi_{r_1}^F$ exhibits a mixture of forward and inverse cascade. Finally at TU, $d U_1<0$ away from the wall for large separations (due to the growth of the boundary layer thickness), while again $\phi_{r_1}^F$ does not exhibit a clear behaviour. It is evident therefore, that at least in the earlier stages of transition, a strong inverse cascade process exists, which is predominately due to the non-linear interaction term. 

\section{Energy fluxes in the $(r_1,r_3)$ plane}\label{sec:fluxes-r1-r3}

In figure \ref{fig:r1r3_peakheight} maps of the scale energy flux vectors $\left(\boldsymbol{\phi_r}_1,\boldsymbol{\phi_r}_3\right)$ in the $(r_1, r_3)$ plane at 4 streamwise locations are shown; the wall normal distances correspond to the peak $\mathcal{P}_{net}$ of figure \ref{r3_flux}. Contours of the net energy production are also superimposed. The panel at location TR1 confirms the strong inverse cascade at regions of high $\mathcal{P}_{net}$, between $5<r_3/L_0<15$. It is clear that the inverse cascade is mainly directed towards the $r_1$ direction; in the $r_3$ direction it appears only for $r_3/L_0>10$, in agreement with figure \ref{r3_flux}, but it is much weaker. A  recirculation pattern in the flow of energy is also evident, i.e.\ energy emanating from the large net production region flows to large $r_1$ and then recirculates back to small $r_1$ and $r_3$ scales. This recirculation look is much more clear in locations TR2 and TU. In TR3 it is not so evident, possibly because of the narrow range of the $r_1$ and $r_3$ separations considered. 

\begin{figure} 
    \centering
     \includegraphics[scale=0.48]{Chapter5_paper2/r1r3_crosspeak_2.png}
    \caption{Scale energy flux vectors $\left(\boldsymbol{\phi_r}_1,\boldsymbol{\phi_r}_3\right)$ on $(r_1, r_3)$ plane at $Y/L_0=5$ for $TR1$ and $TR2$; $Y/L_0=1.3$ for $TR3$ and $TU$ (red arrows). Contour plots of net production are superimposed. The maximum vector magnitude (corresponding to the longest arrow on each plot) is $4.5\times10^{-4}, 1\times10^{-3}, 6\times10^{-4}, 7\times10^{-4}$ from $TR1$ to $TU$ respectively.}
    \label{fig:r1r3_peakheight}
\end{figure}

\section{Maps of energy flux in the 3D ($r_1,r_3,Y$) hyper-plane}\label{sec:fluxes-r1-r3-Y}

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{Chapter5_paper2/LA_3D.png}
    \includegraphics[scale=0.448]{Chapter5_paper2/TR2_3D.png}
    \includegraphics[scale=0.45]{Chapter5_paper2/TU_3D.png}
    \caption{Maps of energy flux in the 3D ($r_1,r_3,Y$) hyper-plane in the form of stream-tubes for 3 streamwise locations. The yellow isosurface denotes  $0.7\max\left(\mathcal{P}_{net}\right)$. The stream-tubes are coloured according to the sign of $\phi_{r_1}$ (red for positive, blue for negative, thus indicating inverse and forward cascade respectively).  The colour bar refers to the value of $\phi_{r_1}$. The radius of the tubes grows with increasing magnitude of the flux vector. Each plot was generated by placing a sphere at a specific location and tracing the stream-tubes crossing the sphere. For $LA$, a sphere of radius $15L_0$ is placed at $(r_1=5L_0, r_3=7.5L_0, Y=5L_0)$ (left and right column show the same stream-tubes from different angles); 
    For $TR2$, a sphere of radius $30L_0$ is placed at two points $(r_1=20L_0 \mbox{ and } 70L_0, r_3=7.5L_0, Y=5L_0)$ (left column) and at $(r_1=70L_0, r_3=7.5L_0, Y=5L_0)$ (right column). For $TU$, a sphere of radius $30L_0$ is placed at two points $(r_1=10L_0 \mbox{ and } 60L_0, r_3=7.5L_0, Y=1.3L_0)$ (left column) and at $(r_1=60L_0, r_3=7.5L_0, Y=1.3L_0)$(right column).}
    \label{KHMH3D}
\end{figure}

In the previous sections we examined the evolution of the energy fluxes on the 2D planes $(r_3,Y), (r_1,Y)$ and $(r_1,r_3)$. The most significant finding is that during the transition, a strong inverse cascade of energy exists that originates from the net production peak region and is mainly directed along the $r_1$ direction. However, previous results provide only limited understanding because they are visualised on 2D planes, so in this section, we map the energy paths on the 3D hyper-plane ($r_1,r_3, Y$). These maps are shown in figure \ref{KHMH3D} for three streamwise locations $LA, TR2 \mbox{ and } TU$, and are visualised from two different viewing angles. To aid understanding, we also superimpose the isosurface $0.7\max\left(\mathcal{P}_{net}\right)$ in yellow colour.  For $TR2 \mbox{ and }TU$ we focus on different areas of the map; we do this by plotting the stream-tubes crossing small spheres placed at different $r_1$ separations (refer to the figure legend for more details).   

In the laminar ($LA$) and transition regions ($TR2$), the net production region (in yellow colour) is centred at $r_3=10L_0, Y=5L_0$ and is elongated in the $r_1$ direction. At $TU$, this region moves closer to the wall ($r_3=5L_0, Y=1.3L_0$) and significantly shrinks in the streamwise direction $(r_1)$. In all three locations, energy stream-tubes emanate from the production region but their behaviour is different. In the laminar ($LA$) region, a weak inverse cascade along the $r_1$ direction is observed and then the flow energy pathlines bend upwards to the bulk of the flow and downwards to the wall region. At $TR2$, the energy flux is an order of magnitude larger compared to $LA$. Very strong inverse cascade is present in the $r_1$ direction, consistent with figures \ref{fig:r1Y_crosspeak} and \ref{fig:r1r3_peakheight}, but the energy paths then bend back to small $r_1$ and $r_3$ and towards the bulk of the flow; this explains the recirculating pattern noticed in figure \ref{fig:r1r3_peakheight}. In the turbulent $TU$ region, there is still inverse cascade in the $r_1$ direction, but it is weaker and confined to a smaller $r_1$ domain. Again, once energy has travelled for a sufficient distance in the $r_1$ direction, the stream-tubes bend to smaller $r_1$ and $r_3$ scales and to the bulk of the flow. The flux map at this location is very similar to that of channel flow, refer to \cite{cimarelli2013paths}.

\section{Analysis of instantaneous interscale energy fluxes in physical space}\label{sec:instantaneous}

\begin{figure} 
    \centering
  \includegraphics[scale=0.6]{Chapter5_paper2/time_ser.PNG}
    \caption{Contour plots of the instantaneous wall-normal velocity fluctuation at $Y=1.3L_0$ at four time instances. The time separation $d t$ between two snapshots is 500 time units.}
    \label{ins_v}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.43]{Chapter5_paper2/ins_Y13_u_whole4.PNG}
%      \includegraphics[scale=0.66]{Fig/ins_Y13_u_whole5.PNG}
%        \includegraphics[scale=0.54]{Fig/ins_Y13_u_whole6.PNG}
    \caption{Contour plots of the instantaneous streamwise velocity fluctuations within the rectangular area marked with a green border in panel (c) of figure \ref{ins_v}. }
    \label{ins95_2}
\end{figure}

The analysis presented in the previous sections identified a strong inverse cascade close to the wall, at wall-normal locations $Y<10L_0$, which is mainly directed in the streamwise direction. In this section, we relate the energy transfer to the physical processes that take place during transition, and in particular to the growth of turbulent spots. 

Figure \ref{ins_v} shows four snapshots of the instantaneous wall-normal velocity fluctuation at $Y=1.3L_0$; the time delay between two snapshots is $d t=500$ time units. In panel $(a)$, two turbulent patches are starting to form at locations $(X-X_0)/L_0 \approx 1300$ and $1400$. The two patches grow and propagate downstream as shown in panel $(b)$, and finally merge to form a large turbulent patch, which is clearly visible in panel $(c)$. This large patch then propagates as a single entity, see panel $(d)$. 

We now focus our attention to the rectangular area marked with a green dashed line in panel $(c)$, which contains both laminar and turbulent regions. This area extends between $1002-1502$ and $0-50$ in the streamwise and spanwise directions respectively, and covers the region between locations $TR1$ and $TR2$ (see markings at the bottom of panel d). In figure \ref{ins95_2} contour plots of the streamwise velocity fluctuations within the selected rectangular area are shown. We chose now two points, one red (at $(X-X_0)/L_0=1252$, within a laminar Klebanoff streak), and one green (at $(X-X_0)/L_0=1402$, within a streak that breaks down). We think of these two points as fixed middle points around which we consider separations $r_1$ up to $150L_0$ (consistent with figure \ref{fig:r1Y_crosspeak}) and $r_3$ up to $50L_0$. These separations define two regions, $[1177,1327]\times[0,50]$ and $[1327,1477]\times[0,50]$, that are marked with dashed yellow and black borders respectively  in figure \ref{ins95_2}.

We can investigate the relation between the instantaneous flow and the scale fluxes within these two regions by plotting them in two separate figures. However the interpretation of the results is facilitated if the two figures are superimposed on a single plot. We do this on the left panel of figure \ref{ins95_3} for the first region $[1177,1327]\times[0,50]$. In this panel, we superimpose the inter-scale energy flux vector $\left(\boldsymbol{\phi_r}_1, \boldsymbol{\phi_r}_3\right)$ on the $(r_1, r_3)$ plane (top and right axes) together with the instantaneous streamwise fluctuations in the $(X,Z)$ plane (left and bottom axes). The process is as follows: we select an arbitrary point $x_i^{+}=X_i + r_i/2$ to the right of the middle point $X_i$, and find the corresponding $x_i^{-}=X_i - r_i/2$, as shown in the figure. We then compute the energy flux vector using the fluctuations in these two points, and place the vector at $x_i^{+}$ (and since $x_i^+=X_i+r_i/2$, the legends of the top and right axes are $r_1/(2L_0)$ and $r_3/(2L_0)$ respectively). In this way we can relate directly the instantaneous inter-scale energy fluxes with the dynamics of the streak breakdown and turbulent patch formation and growth. The right boundary of the area considered in figure \ref{ins95_3} is just upstream of the streak breakdown, see also figure \ref{ins95_2}. Note the stronger streamwise velocity fluctuations when the two high speed streaks start to break down (at $Z/L_0 \approx 10$ and $\approx 30$) and the associated inverse cascade.  Forward cascade is observed instantaneously around the narrow low speed streak located in between, at $Z/L_0 \approx 20$. In the right panel, we present both the flux vectors and contours of the flux component $\boldsymbol{\phi_r}_1$; the contours show that the inverse cascade is relatively week at this time instant and location. 

\begin{figure}
    \centering
\includegraphics[scale=0.43]{Chapter5_paper2/ins_Y13_both_beforespots4.PNG}
\caption{Contours of the streamwise velocity fluctuations (left) and of the energy flux component $\boldsymbol{\phi_r}_1$ (right). In both panels, the superposed black arrows indicate the direction of the energy flux vector $\left(\boldsymbol{\phi_r}_1, \boldsymbol{\phi_r}_3\right)$. The middle point is located at $(X-X_0)/L_0=1252$.} 
\label{ins95_3}
\end{figure}


\begin{figure} 
    \centering
\includegraphics[scale=0.6]{Chapter5_paper2/ins_Y13_both_withinspots5.PNG}
    \caption{Contours of the streamwise velocity fluctuations (left) and of the energy flux component $\boldsymbol{\phi_r}_1$ (right). In both panels, the superposed black arrows indicate the direction of the energy flux vector $\left(\boldsymbol{\phi_r}_1, \boldsymbol{\phi_r}_3\right)$. The middle point is located at $(X-X_0)/L_0=1402$.} 
    \label{ins95_4}
\end{figure}

We repeat the process for the region marked by the black border in figure \ref{ins95_2}. The middle point is now at $(X-X_0)/L_0=1402$ and is located firmly within the streak break down region; indeed it is surrounded by two high speed streaks that disintegrate to form a turbulent spot; the spot can be clearly seen  in panel (c) of figure \ref{ins_v}. The results, shown in figure \ref{ins95_4}, indicate that the large velocity fluctuations inside the streaks contribute to an inverse cascade around the middle point, and this corresponds to the growth of the high-speed streaks within the turbulent spot. Comparison of the streamwise flux components $\boldsymbol{\phi_r}_1$ (right panels of figures \ref{ins95_3} and \ref{ins95_4}) shows that the inverse cascade is much stronger when the streaks breakdown. This is because the inter-scale flux scales with the cube of velocity difference, so a small increase in $d u_1$ results in much larger fluxes.

In both regions considered, inverse cascade appears when the instantaneous flow accelerates between $x_i^-$ to $x_i^+$. This can also  seen in the average picture in figure \ref{fig:r1Y_crosspeak}.
\begin{figure}
    \centering
     \includegraphics[scale=0.5]{Chapter5_paper2/PDF_1.png}
     \includegraphics[scale=0.5]{Chapter5_paper2/PDF_2.png} 
     \includegraphics[scale=0.5]{Chapter5_paper2/PDF_3.png}
    \caption{PDFs of $\boldsymbol{\phi_{r_1}}$ (top) with the Mean (middle) and fluctuating (bottom) components at $TR1$ location for $(r_1=50L_0,r_2=0.r_3=8L_0)$.}
    \label{fig:PDF_TR1_raw_data}
\end{figure}
Note that the interpretation of inverse cascade for fixed values of $r_3$ (for example for those values where $\mathcal{P}_{net}$ is maximised, as in figure \ref{r1_flux_decom_crosspeak}) refers to the growth of streaks within spots. This is of course related to the growth of spots themselves, as the latter consist of high-speed streaks that grow individually. 

The analysis of the growth of spots as single entities in the spanwise direction using the KHMH formulation is possible, but it is more involved. It would require the identification of a spot using an indicator function as in \cite{marxen2019turbulence,Yao_Portela_Papadakis_2020}, positioning of the midpoint $X_i$ at the centroid of the spot, and integration of the KHMH equation in the scale space around the spot bounding surface. This is a generalisation of the integration over a sphere performed by \cite{hill2002exact} and can elucidate very clearly the mechanisms for interscale energy transfer to the spot as a single entity. This is however beyond the scope of the present paper. 

The previous analysis demonstrated that the scale fluxes depend strongly on the distance from the wall and are  highly intermittent. This motivates the investigation of their probability density function (PDF). Figure \ref{fig:PDF_TR1_raw_data} shows the PDF of $\boldsymbol{\phi_{r_1}}$ (top panel) at the streamwise location $TR1$ for fixed separation  $(r_1,r_3)=(50L_0,8L_0)$ and three different wall-normal distances. We also plot the PDFs of the components $\phi_{r_1}^M= d U_1 d q^2 $ (mid panel) and $\phi_{r_1}^F= d u_1 d q^2 $ (bottom panel). In total $55,000$ time and spanwise samples  were used to construct these PDFs.  Although this is not ideal, because spanwise samples smooth out the fluxes around localised spots shown in figures \ref{ins_v}, the PDFs still provide a more complete picture compared to time-averages.   %We have used $351\times157 \approx 55,000$ samples to construct these PDF's. 

At the separations considered there is strong inverse cascade, as shown in figure \ref{fig:r1Y_crosspeak}. At $Y=7L_0$, where the inverse cascade is  maximised, the shape of the PDF of $\boldsymbol{\phi_{r_1}}$ is slightly asymmetric and skewed towards positive values. At the other two locations, the PDF is nearly symmetric resulting in very low time-averages. The PDFs of  $\phi_{r_1}^M$ are one-sided; the sign depends on $d U_1$ and varies with wall-normal distance. This results in a competition between  $\phi_{r_1}^F$ and $\phi_{r_1}^M$ in the core of the boundary layer. However, $\phi_{r_1}^M$ attains small values, and the overall effect on $\boldsymbol{\phi_{r_1}}$ is small. Note the presence of rare (low probability) but very strong positive and negative fluxes of $\phi_{r_1}^F$ at $Y=7L_0$. Similar behavior has been observed for the PDFs of fluxes in homogeneous isotropic turbulence, see figure 3 in \cite{yasuda2018spatio} and also \cite{Ishihara_et_al_2009,Aoyama_et_al_2005}, but in this case the time-average is negative (standard forward cascade). Therefore the presence of turbulent spots in a transitional flow modifies the average picture, even though the results are spanwise- averaged and the localised spot effect is diluted; this indicates that it must be quite strong. The rare positive and negative events are still there, and it is not clear how the the two forms of intermittency, one due to small-scale structures present in turbulent flows and the other due to transition, interact. This motivates a more careful analysis of interscale fluxes, for example one in which the fluxes are conditioned on the flow state (laminar or turbulent) at points $x_i^+$ and $x_i^-$. Such conditional analysis has been performed by \cite{Yao_Portela_Papadakis_2020} for the second-order structure functions and can be extended to interscale fluxes as well; we leave this for future work.

\section{Conclusions}\label{sec:conclusions}
We apply the KHMH equation to analyse the interscale energy flux in a flat plate boundary layer undergoing bypass transition due to forcing from free-stream turbulence. Energy from the mean flow is injected at a particular spanwise length scale and wall-normal position, both of which are determined by the interaction between the external forcing and the mean shear (linear receptivity process) that takes place in the early development of the boundary layer. From this production peak, energy fluxes radiate to different directions in physical and scale spaces. Two- and three-dimensional flux maps in the transitional regime show a very strong inverse cascade near the wall (i.e.\ energy flows from small to large scales) in the streamwise direction. Analysis of the constituent components of the total flux indicates that the inverse cascade is due to the non-linear interactions between velocity fluctuations. Other components, such as the one due to mean flow inhomogeneity, are non-negligible, but are not strong enough to affect the flux direction. As the transition process approaches completion, the maps morph to those encountered in other fully developed turbulent flows, such as channel flow, where there is weak inverse cascade in the streamwise direction, and then then flux vectors bend towards small scales.

Superposition of the instantaneous flux vectors with the corresponding flow fields relates the cascade process to the growth of turbulent structures in the streamwise direction. The sign of the time and spanwise- average flux is positive across the boundary layer thickness and this is related to predominantly accelerating events that lead to the elongation of vortex structures within a spot, and consequently to the spot itself. The probability density function of the flux is asymmetric and skewed towards positive values. However, strong but rare forward and inverse cascade events are present, as in homogeneous isotropic turbulence. 

The present results have painted a picture of interscale transfer in transitional flows that deviates significantly from that of fully developed, wall-bounded, turbulent flows. Spanwise averaging dilutes the transfer process within  nascent and developing spots, as a large proportion of the flow remains laminar in the early stages of transition. More in depth investigations using conditional averaging, an operation that naturally accounts for intermittency effects due to transition, are certainly warranted. Such investigations will elucidate the contributions to the average interscale transfer arising from different events, i.e.\ when the points $x_i^+$ and $x_i^-$ are both located in laminar or turbulent patches, or one is placed in a laminar and the other in a turbulent region. The Conditional KHMH analysis will be presented in the following section.



%\section{Yao, H., J.-P. Mollicone and Papadakis, G. 2021 Analysis of interscale energy transfer in a boundary layer undergoing bypass transition. \textit{Journal of Fluid Mechanics}, (submitted).}

%\includepdf[pages=-]{Chapter5_paper2/Paper_2.pdf}
